PreViTS: Contrastive Pretraining with Video Tracking Supervision

Videos are a rich source for self-supervised learning (SSL) of visual representations due to the presence of natural temporal transformations of objects. However, current methods typically randomly sample video clips for learning, which results in an imperfect supervisory signal. In this work, we propose PreViTS, an SSL framework that utilizes an unsupervised tracking signal for selecting clips containing the same object, which helps better utilize temporal transformations of objects. PreViTS further uses the tracking signal to spatially constrain the frame regions to learn from and trains the model to locate meaningful objects by providing supervision on Grad-CAM attention maps. To evaluate our approach, we train a momentum contrastive (MoCo) encoder on VGG-Sound and Kinetics-400 datasets with PreViTS. Training with PreViTS outperforms representations learnt by contrastive strategy alone on video downstream tasks, obtaining state-of-the-art performance on action classification. PreViTS helps learn feature representations that are more robust to changes in background and context, as seen by experiments on datasets with background changes. Learning from large-scale videos with PreViTS could lead to more accurate and robust visual feature representations.

==> figures/constrained_cropping.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/constrained_cropping.png}
    \caption{Cropping align the same object by video object segmetation supervision (slot filler)}
    \label{fig:constrained_cropping}

\end{figure}

==> figures/predict_trans.tex <==
\begin{figure}[t]
    
    \includegraphics[width=0.5\textwidth]{figures/predict_trans.png}
    \caption{Predict transformation of the middle segment (slot filler)}
    \label{fig:predict_trans}

\end{figure}

==> figures/random_crop.tex <==
\begin{figure}[t]
    
    \includegraphics[width=0.5\textwidth]{figures/random_crop.png}
    
    \caption{random cropping may leads to different concept (slot filler)}
    \label{fig:random_crop}

\end{figure}

==> sup/super_mask.tex <==
\begin{table}[t]
    \centering \scriptsize
    \setlength{\tabcolsep}{2pt}
%\begin{subfigure}[t]{0.6\linewidth}
        \begin{tabularx}{0.7\linewidth}{lXccc}
        \toprule
        \textbf{Tracking supervision} &&No Tracking& Unsupervised & Supervised \\
        \midrule
        \textbf{\vocclf{}} && 68.3\Drop{4.7} &\graycell 73.0 &  75.0 \Rise{2.0} \\
        %\textbf{\ucf{}} && 79.0  \Drop{5.5} &\graycell 84.5  & 86.1 \Rise{1.6} \\
        \bottomrule
        \end{tabularx}
        %\vspace{-2pt}
        %\caption{\scriptsize Effect of different tracking supervision}
        
        \vspace{+5pt}
    %\end{subfigure}
    
    \caption{
        \textbf{Effect of different tracking supervision.} Replacing unsupervised video tracking supervision with supervised tracking improves downstream performance slightly.
        \label{subtab:ablations3}
    }   
    %\label{tab:train_ablations}
    %\vspace{-10pt}
\end{table}

==> tables/video_bg.tex <==
\begin{table*}[t]

    \newcolumntype{Y}{>{\raggedright\arraybackslash}X}
    \newcolumntype{Z}{>{\centering\arraybackslash}X}

    \centering
    \footnotesize
    %\setlength\tabcolsep{1pt}
    \renewcommand{\arraystretch}{1.2}

    \begin{tabularx}{\textwidth}{ p{0.15\textwidth} c llllllll}
    \toprule
    \multicolumn{1}{l}{\bf \multirow[b]{2}{*}{\makecell{RSPNet-K400\\ Performance}}}
    & 
    & \multicolumn{8}{c}{\bf Video Backgrounds Challenge }\\
    \cmidrule{3-10} 
     ~ &  ~& Original & \makecell{Mixed-Same}  & \makecell{Mixed-Rand}  & \makecell{Mixed-Next} &   \makecell{Only-FG}  &
     \makecell{No-FG}  & \makecell{Only-BG-B}  &  \makecell{Only-BG-T}    \\
    \midrule
     \band
    Default &~& 70.7 & 40.7 & 30.3 & 29.5 & 20.9 & 49.1  &  35.2 & 28.6  \\
    \app{}   &~&      74.0\Rise{3.3}   &  48.0\Rise{7.3}     & 35.9~\Rise{5.6}    & 32.7\Rise{3.2}    &  27.8\Rise{6.9}   & 51.9\Rise{2.8}   &  33.7\Riseneg{1.5}    &  28.3\riseneg{0.3}   \\
    \bottomrule
    \end{tabularx}
    \caption{\app{} achieved significant improvements over RSPNet on the Video Backgrounds Challenge. We observe a similar trend as the Image Background Challenge, which demonstrates that our model can generalize to videos and robust to background changes. We also found Only-FG to be challenging in video tasks since all of the foregrounds are human.}
    
    \label{tab:backgrounds_results_vid}
    
\end{table*}



==> tables/video_bg2.tex <==
\begin{table}[h]
    \newcommand{\apbbox}[1]{AP$^\text{bbox}_\text{#1}$}
    \newcommand{\apmask}[1]{AP$^\text{mask}_\text{#1}$}
    \newcolumntype{Y}{>{\raggedright\arraybackslash}X}
    \newcolumntype{Z}{>{\centering\arraybackslash}X}

    \centering
    \footnotesize
    \setlength\tabcolsep{1pt}
    \renewcommand{\arraystretch}{1.2}

    \begin{tabular}[]{lcccc}
        \toprule
        \textbf{RSPNet-K400} && Original && No-FG  \\
        \midrule
        \textbf{Default} && 47.18 && 44.47 \\
        \textbf{\app} && 55.24  &&  48.34   \\
        \bottomrule
        \end{tabular}
        %\vspace{-3pt}
        %\caption{Effect of improving underlying \mocococo{}}
        \label{tab:davis}
        %\vspace{5pt}
    %\vspace{-5pt}
    \caption{\textbf{Video Background Challenge:} Mini-Kinetics
    } 
    \label{tab:video_back_dance}
    %\vspace{-15pt}
\end{table}


==> temp/definitions.tex <==
% DB: got tired of typing braces
\newcommand{\haty}{\hat{y}}

% shortcuts for bots
\newcommand{\Qbot}{\textsc{Q-bot}\xspace}
\newcommand{\Abot}{\textsc{A-bot}\xspace}

\newcommand{\vd}{VisDial\xspace}
\newcommand{\vdfull}{Visual \Dialog}
\newcommand{\vqa}{VQA\xspace}

% consistent formatting for quoting in the paper
\newcommand{\myquote}[1]{\emph{`#1'}}
\newcommand{\myapprox}{{\raise.17ex\hbox{$\scriptstyle\sim$}}}
% consistent bold starts
\newcommand{\xhdr}[1]{\vspace{2pt}\noindent\textbf{#1}}

% environment for margin change
\def\changemargin#1#2{\list{}{\rightmargin#2\leftmargin#1}\item[]}
\let\endchangemargin=\endlist 

% Definitions for referring to figure, section, table, equation
% (used uniformly thoughout)
\newcommand{\reffig}[1]{Figure~\ref{#1}}
\newcommand{\refsec}[1]{Sec.~\ref{#1}}
\newcommand{\reftab}[1]{Tab.~\ref{#1}}
%\newcommand{\refeq}[1]{Eq.~\ref{#1}}

% train, val, test
\newcommand{\train}{\texttt{train}\xspace}
\newcommand{\val}{\texttt{val}\xspace}
\newcommand{\test}{\texttt{test}\xspace}

% shortcuts for embodied QA
\newcommand{\eqafull}{Embodied Question Answering\xspace}
%\newcommand{\eqa}{EQA\xspace}
%\newcommand{\eqa}{\textsc{EmbodiedQA}\xspace}
%\newcommand{\eqa}{EmbodiedQA\xspace}
%\newcommand{\eqa}{\textsc{EmbodQA}\xspace}
%\newcommand{\eqa}{\textsc{EQA}\xspace}
\newcommand{\eqa}{EmbodiedQA\xspace}
\newcommand{\hierEQA}{\texttt{Hier-EQA~}}
%\newcommand{\act}{\texttt{ACT-EQA~}}
\newcommand{\eqads}{EQA\xspace}


%\DeclareMathOperator*{\argmin}{arg\,min}
%\DeclareMathOperator*{\argmax}{arg\,max}
\def\support{\mbox{support}}
%% Italian Short Terms
\def\diag{\mbox{diag}}
\def\rank{\mbox{rank}}
\def\grad{\mbox{\text{grad}}}
\def\dist{\mbox{dist}}
\def\sgn{\mbox{sgn}}
\def\tr{\mbox{tr}}
\def\etal{\textit{et al}.~}
\def\card{{\mbox{Card}}}
\def\ie{\mbox{\textit{i.e.}, }}
\def\eg{\mbox{\textit{e.g.}, }}
\def\wrt{\mbox{\textit{w.r.t. }}}
\def\vol{{\mbox{vol}}}
\def\diam{\mbox{diam}}

%%bold greek letters\bvarpi
\def\balpha{\mbox{{\boldmath $\alpha$}}}
\def\bbeta{\mbox{{\boldmath $\beta$}}}
\def\bzeta{\mbox{{\boldmath $\zeta$}}}
\def\bgamma{\mbox{{\boldmath $\gamma$}}}
\def\bdelta{\mbox{{\boldmath $\delta$}}}
\def\bmu{\mbox{{\boldmath $\mu$}}}
\def\bftau{\mbox{{\boldmath $\tau$}}}
\def\beps{\mbox{{\boldmath $\epsilon$}}}
\def\blambda{\mbox{{\boldmath $\lambda$}}}
\def\bLambda{\mbox{{\boldmath $\Lambda$}}}
\def\bnu{\mbox{{\boldmath $\nu$}}}
\def\bomega{\mbox{{\boldmath $\omega$}}}
\def\bfeta{\mbox{{\boldmath $\eta$}}}
\def\bsigma{\mbox{{\boldmath $\sigma$}}}
\def\bzeta{\mbox{{\boldmath $\zeta$}}}
\def\bphi{\mbox{{\boldmath $\phi$}}}
\def\bxi{\mbox{{\boldmath $\xi$}}}
\def\bvphi{\mbox{{\boldmath $\phi$}}}
\def\bdelta{\mbox{{\boldmath $\delta$}}}
\def\bvarpi{\mbox{{\boldmath $\varpi$}}}
\def\bvarsigma{\mbox{{\boldmath $\varsigma$}}}
\def\bXi{\mbox{{\boldmath $\Xi$}}}
\def\bmW{\mbox{{\boldmath $\mW$}}}
\def\bmY{\mbox{{\boldmath $\mY$}}}

\def\bPi{\mbox{{\boldmath $\Pi$}}}

\def\bOmega{\mbox{{\boldmath $\Omega$}}}
\def\bDelta{\mbox{{\boldmath $\Delta$}}}
\def\bPi{\mbox{{\boldmath $\Pi$}}}
\def\bPsi{\mbox{{\boldmath $\Psi$}}}
\def\bSigma{\mbox{{\boldmath $\Sigma$}}}
\def\bUpsilon{\mbox{{\boldmath $\Upsilon$}}}

%%mathcal letters
\def\mA{{\mathcal A}}
\def\mB{{\mathcal B}}
\def\mC{{\mathcal C}}
\def\mD{{\mathcal D}}
\def\mE{{\mathcal E}}
\def\mF{{\mathcal F}}
\def\mG{{\mathcal G}}
\def\mH{{\mathcal H}}
\def\mI{{\mathcal I}}
\def\mJ{{\mathcal J}}
\def\mK{{\mathcal K}}
\def\mL{{\mathcal L}}
\def\mM{{\mathcal M}}
\def\mN{{\mathcal N}}
\def\mO{{\mathcal O}}
\def\mP{{\mathcal P}}
\def\mQ{{\mathcal Q}}
\def\mR{{\mathcal R}}
\def\mS{{\mathcal S}}
\def\mT{{\mathcal T}}
\def\mU{{\mathcal U}}
\def\mV{{\mathcal V}}
\def\mW{{\mathcal W}}
\def\mX{{\mathcal X}}
\def\mY{{\mathcal Y}}
\def\mZ{{\mathcal{Z}}}


%%bold mathcal letters
\DeclareMathAlphabet\mathbfcal{OMS}{cmsy}{b}{n}
%bold mathcal letters

\def\bmA{{\mathbfcal A}}
\def\bmB{{\mathbfcal B}}
\def\bmC{{\mathbfcal C}}
\def\bmD{{\mathbfcal D}}
\def\bmE{{\mathbfcal E}}
\def\bmF{{\mathbfcal F}}
\def\bmG{{\mathbfcal G}}
\def\bmH{{\mathbfcal H}}
\def\bmI{{\mathbfcal I}}
\def\bmJ{{\mathbfcal J}}
\def\bmK{{\mathbfcal K}}
\def\bmL{{\mathbfcal L}}
\def\bmM{{\mathbfcal M}}
\def\bmN{{\mathbfcal N}}
\def\bmO{{\mathbfcal O}}
\def\bmP{{\mathbfcal P}}
\def\bmQ{{\mathbfcal Q}}
\def\bmR{{\mathbfcal R}}
\def\bmS{{\mathbfcal S}}
\def\bmT{{\mathbfcal T}}
\def\bmU{{\mathbfcal U}}
\def\bmV{{\mathbfcal V}}
\def\bmW{{\mathbfcal W}}
\def\bmX{{\mathbfcal X}}
\def\bmY{{\mathbfcal Y}}
\def\bmZ{{\mathbfcal Z}}

%%bold letters
\def\0{{\bf 0}}
% \def\1{{\bf 1}}
\usepackage{ dsfont }
\def\1{\mathds{1}}

%%bold capital Cases
\def\bA{{\bf A}}
\def\bB{{\bf B}}
\def\bC{{\bf C}}
\def\bD{{\bf D}}
\def\bE{{\bf E}}
\def\bF{{\bf F}}
\def\bG{{\bf G}}
\def\bH{{\bf H}}
\def\bI{{\bf I}}
\def\bJ{{\bf J}}
\def\bK{{\bf K}}
\def\bL{{\bf L}}
\def\bM{{\bf M}}
\def\bN{{\bf N}}
\def\bO{{\bf O}}
\def\bP{{\bf P}}
\def\bQ{{\bf Q}}
\def\bR{{\bf R}}
\def\bS{{\bf S}}
\def\bT{{\bf T}}
\def\bU{{\bf U}}
\def\bV{{\bf V}}
\def\bW{{\bf W}}
\def\bX{{\bf X}}
\def\bY{{\bf Y}}
\def\bZ{{\bf{Z}}}

%%bold small cases
\def\ba{{\bf a}}
\def\bb{{\bf b}}
\def\bc{{\bf c}}
\def\bd{{\bf d}}
\def\be{{\bf e}}
\def\bff{{\bf f}}
\def\bg{{\bf g}}
\def\bh{{\bf h}}
\def\bi{{\bf i}}
\def\bj{{\bf j}}
\def\bk{{\bf k}}
\def\bl{{\bf l}}
\def\bm{{\bf m}}
\def\bn{{\bf n}}
\def\bo{{\bf o}}
\def\bp{{\bf p}}
\def\bq{{\bf q}}
\def\br{{\bf r}}
\def\bs{{\bf s}}
\def\bt{{\bf t}}
\def\bu{{\bf u}}
\def\bv{{\bf v}}
\def\bw{{\bf w}}
\def\bx{{\bf x}}
\def\by{{\bf y}}
\def\bz{{\bf z}}

%%hat letters
\def\hy{\hat{y}}
\def\hby{\hat{{\bf y}}}


%%mathrm letters
\def\mmE{{\mathbb E}}
\def\mmP{{\mathbb P}}
\def\mmQ{{\mathbb Q}}
\def\mmB{{\mathrm B}}
\def\mmR{{\mathbb R}}
\def\mmS{{\mathbb S}}
\def\mmV{{\mathbb V}}
\def\mmN{{\mathbb N}}
\def\mmZ{{\mathbb Z}}
\def\mMLr{{\mM_{\leq k}}}

%%tidle cases
\def\tC{\tilde{C}}
\def\tk{\tilde{r}}
\def\tJ{\tilde{J}}
\def\tbx{\tilde{\bx}}
\def\tbK{\tilde{\bK}}
\def\tL{\tilde{L}}
\def\tbPi{\mbox{{\boldmath $\tilde{\Pi}$}}}
\def\tw{{\bf \tilde{w}}}

%%bar cases
\def\barx{\bar{\bx}}

%%terms for short
\def\pd{{\succ\0}}
\def\psd{{\succeq\0}}
\def\vphi{\varphi}
\def\trsp{{\sf T}}

%short phrase
\def\mRMD{{\mathrm{D}}}
\def \DKL{{D_{KL}}}
\def\st{{\mathrm{s.t.}}}
\def\nth{{\mathrm{th}}}
\def\Pr{{\mathrm{Pr}}}
\def\patch{{\mathrm{patch}}}

\def\bx{{\bf x}}
\def\bX{{\bf X}}
\def\by{{\bf y}}
\def\bY{{\bf Y}}
\def\bw{{\bf w}}
\def\bW{{\bf W}}
\def\balpha{{\bm \alpha}}
\def\bbeta{{\bm \beta}}
\def\boldeta{{\bm \eta}}
\def\boldEta{{\bm \Eta}}
%\def\bgamma{{\bm \gamma}}
\def\bGamma{{\bm \Gamma}}
\def\bmu{{\bm \mu}}

\def\bK{{\bf K}}
\def\bb{{\bf b}}
\def\bg{{\bf g}}
\def\bp{{\bf p}}
\def\bP{{\bf P}}
\def\bh{{\bf h}}
\def\bc{{\bf c}}
\def\bz{{\bf z}}

\def\st{{\mathrm{s.t.}}}
\def\tr{\mathrm{tr}}
\def\grad{{\mathrm{grad}}}
\def\Id{{\mathrm{Id}}}

\usepackage{ntheorem}
\newtheorem{coll}{Corollary}
\newtheorem{deftn}{Definition}
\newtheorem{thm}{Theorem}
\newtheorem*{*thm}{Theorem}
\newtheorem{prop}{Proposition}
%\newtheorem{lemma}{Lemma}
\newtheorem*{*lemma}{Lemma}
%\newtheorem{remark}{Remark}
\newtheorem{ass}{Assumption}
\newtheorem{prob}{Problem}
%\newtheorem*{proof}{Proof}
%\newenvironment*{proof}{\textbf{Proof}\quad}{\hfill $\square$\par}
\renewcommand\theprob{\Roman{prob}}

\usepackage{enumitem}
\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}  
\newcommand{\yes}{\textcolor[rgb]{0,0.6,0}{\large{\checkmark}}}
\newcommand{\no}{\textcolor[rgb]{0.6,0,0}{\large{{\bf\times}}}}

\def\red{\textcolor{red}}
\def\blue{\textcolor{blue}}
\def\green{\textcolor{green}}

